Strongly refuting all semi-random Boolean CSPs

We give an efficient algorithm to strongly refute \emph{semi-random} instances of all Boolean constraint satisfaction problems. The number of constraints required by our algorithm matches (up to polylogarithmic factors) the best-known bounds for efficient refutation of fully random instances. Our main technical contribution is an algorithm to strongly refute semi-random instances of the Boolean $k$-XOR problem on $n$ variables that have $\widetilde{O}(n^{k/2})$ constraints. (In a semi-random $k$-XOR instance, the equations can be arbitrary and only the right-hand sides are random.) One of our key insights is to identify a simple combinatorial property of random XOR instances that makes spectral refutation work. Our approach involves taking an instance that does not satisfy this property (i.e., is \emph{not} pseudorandom) and reducing it to a partitioned collection of $2$-XOR instances. We analyze these subinstances using a carefully chosen quadratic form as a proxy, which in turn is bounded via a combination of spectral methods and semidefinite programming. The analysis of our spectral bounds relies only on an off-the-shelf matrix Bernstein inequality. Even for the purely random case, this leads to a shorter proof compared to the ones in the literature that rely on problem-specific trace-moment computations.

==> content/backup_no_duplicate_edges.tex <==
\begin{theorem}[Degree-bounded Partitioned 2-XOR Refutation]\label{2xor_bounded_partitioned}
	Let $0 < \varepsilon < 1/2$.
	Let $\psi = (V,\ell,E,r)$ be a semirandom partitioned 2-XOR instance with $|V| = n$, $\ell = O(\operatorname{poly}(n))$, and $|E| = m$.
	Additionally assume that $E$ is a set (instead of a multiset), so that each $(i,e)$ appears at most once in $E$.
	Let $0 < d \leq O(\poly(\varepsilon^{-1}, \log n))$, and suppose that for fixed $i \in [\ell]$ and $v \in V$, there are at most $d$ different $(i,e) \in E$ such that $v \in e$.
	Then there is an absolute constant $K$ such that if 
	\[m \geq \max\left\{\frac{Kd n\sqrt{\ell} \log(n)^3}{\varepsilon^{2}}, \frac{\ell}{\varepsilon^2}\right\}\]
	we can with high probability efficiently certify that
	\[\opt(\varphi) \leq 1/2 + \varepsilon.\]
\end{theorem}

Define the set $T_i = \{e \mid (i,e) \in E\}$.
Let $t_i = |T_i|$.
We assume that each partition set $T_i$ is nonempty, as lowering $\ell$ only makes it easier to refute.
Extend the function $r$ by giving all previously undefined inputs a value of zero.
First we define a function $\Phi: \{\pm 1\}^n \to \mathbb{R}$ as follows.
\[\Phi(x) = \sum_{i=1}^\ell \frac{1}{\sqrt{t_i}}\left(\sum_{e \in T_i} x^e r_i(e)\right)^2\]
The following lemma shows that when $\opt(\psi)$ has a large value, $\Phi(x)$ can take on a large value as well.
\begin{lemma}
	If $\opt(\psi) \geq 1/2 + \varepsilon$, then there is $x \in \{\pm 1\}^V$ such that
	\[\Phi(x) \geq \frac{4	\varepsilon^2 m^{3/2}}{\ell^{1/2}}\]
\end{lemma}
\begin{proof}
    Let $(x,y)$ be a maximally satisfying assignment to $\psi$.
	Let $s_i$ be the number of edges in $T_i$ which are satisfied by $(x,y)$.
	Note that $\sum_i s_i \geq (1/2 + \varepsilon)m$, $\sum_i t_i = m$, and
	$\sum_{e \in T_i} x^e r_i(e)y_i = 2s_i - t_i$.
	We use the fact that every $y_i^2 = 1$ to show
	\begin{align*}
	\Phi(x)
	&= \sum_{i = 1}^\ell \frac{1}{\sqrt{t_i}}\left(\sum_{e \in T_i} x^e r_i(e)\right)^2
	= \sum_{i = 1}^\ell \frac{1}{\sqrt{t_i}}\left(\sum_{e \in T_i} x^e r_i(e)y_i\right)^2
	= \sum_{i = 1}^\ell \frac{(2s_i - t_i)^2}{\sqrt{t_i}} \\
	&\geq \frac{\left(\sum_{i=1}^\ell 2s_i - t_i\right)^2}{\sum_{i=1}^\ell \sqrt{t_i}}
	\geq \frac{\big(2(1/2 + \varepsilon)m - m\big)^2}{\sqrt{\ell m}} = \frac{4\varepsilon^2 m^{3/2}}{\ell^{1/2}}
	\end{align*}
where the first inequality follows from Cauchy-Schwarz applied to the sequences $u_i = (2s_i-t_i)/t_i^{1/4}$ and $v_i = t_i^{1/4}$, and the second inequality follows from Cauchy-Schwarz applied to $\sum_i \sqrt{t_i}$, as well as our bounds on $\sum_i s_i$ and $\sum_i t_i$.
\end{proof}
So to show $\opt(\psi) \leq 1/2 + \varepsilon$, it suffices to show $\Phi(x) \leq \frac{4 \varepsilon^2 m^{3/2}}{\ell^{1/2}}$.
Notice that by focusing on bounding $\Phi(x)$, we have effectively removed $y$ from consideration.
Write
\[\Phi(x) = \left(\sum_{i=1}^\ell \frac{1}{\sqrt{t_i}}\sum_{(e, e') \in \binom{T_i}{2}} x^e x^{e'} r_i(e)r_i(e) \right) + \left(\sum_{i=1}^\ell \frac{1}{\sqrt{t_i}} \sum_{e \in T_i} (x^e)^2r_i(e)^2\right)\]
and let $\Phi_1(x)$ be the first term above and $\Phi_2(x)$ be the second.
We bound $\Phi(x)$ by bounding the two terms individually.
\begin{lemma}
	\[\Phi_2(x) \leq \frac{\varepsilon^2 m^{3/2}}{\ell^{1/2}}\]
\end{lemma}
\begin{proof}
	See that every term in the inner summation in $\Phi_2(x)$ is 1, since $r_i(e),x^e \in \{\pm 1\}$.
	Thus the entire inner summation is $t_i$, meaning
	\[\Phi_2(x) = \sum_{i=1}^\ell \sqrt{t_i} \leq \sqrt{\ell \sum_{i=1}^\ell t_i} = \sqrt{\ell m}\]
	where the inequality follows from Cauchy-Schwarz.
	Since $\ell \leq \varepsilon^2 m$ by our lower bound on $m$, we see $\sqrt{\ell m} \leq \frac{\varepsilon^2 m^{3/2}}{\ell^{1/2}}$, completing the proof.
\end{proof}

Thus, if we can prove the following lemma, we will be done.
\begin{lemma}\label{2xor_phi1small}
	With high probability, we can certify that
	\[\Phi_1(x) \leq \frac{\varepsilon^2 m^{3/2}}{\ell^{1/2}}\]
	for all $x \in \{\pm 1\}^n$.
\end{lemma}

The rest of this section is dedicated to proving Lemma~\ref{2xor_phi1small}.
Define $\deg_i(v) = \sum_{u \in V} r_i(v,u)^2$.
Now $r_i(v,u)^2$ is just the 0/1 indicator of $(v,u) \in T_i$, so $\gamma_i(v)$ is just the degree of $v$ in the graph with vertex set $V$ and edge set $T_i$.
Define a function $\gamma:V^2 \to \mathbb{R}$ as follows.
\begin{equation}\label{gamma_defn}\gamma(v,v') = \sum_{i=1}^\ell \frac{\deg_i(v) \deg_i(v')}{t_i}\end{equation}
We refer to $\gamma(v,v')$ as the \emph{weight} of the pair $(v,v')$.
Intuitively, $\gamma(v,v')$ will be high when $v$ and $v'$ have relatively high degrees within relatively small $T_i$.
The next lemma shows that the total weight of all pairs is not too large.
\begin{lemma}\label{2xor_gammasum}
	\[\sum_{v,v' \in [n]} \gamma(v,v') = 4m\]
\end{lemma}
\begin{proof} Indeed,
\begin{align*}
	\sum_{v,v' \in [n]} \gamma(v,v')
	&=  \sum_{i=1}^\ell \frac{1}{t_i} \sum_{v,v' \in V} \deg_i(v) \deg_i(v') \\
	&=  \sum_{i=1}^\ell \frac{1}{t_i} \left(\sum_{v \in V} \deg_i(v)\right)^2
	\end{align*}
	Since $\sum_{v \in V} \deg_i(v) = 2t_i$ and $\sum_i t_i = m$, the lemma follows.
\end{proof}

We now define a partition $S_0, S_1, \dots, S_{\log n}$ of $V^2$ by breaking pairs $(v,v')$ into different ``weight classes''.
We define three numbers $R, \alpha, \beta \in \mathbb{R}$ as follows:
\begin{align}
&R = \frac{Cd^2 \log(n)^6}{\varepsilon^4},
&&\alpha = \frac{R\ell}{4m},
&&&\beta = \left(\frac{4m}{\alpha}\right)^{1/\log n}
\end{align}
Where $C$ is some large enough absolute constant, with the precise meaning of ``large enough'' to be determined later.

We define the sets $S_j$ as follows.
\begin{align*}
	S_0 &= \left\{(v,v') \in V^2 \mid \gamma(v,v') \leq \alpha\right\} \text{ and} \\
	S_j &= \left\{(v,v') \in V^2 \mid \alpha\beta^{j-1} \leq \gamma(v,v') \leq \alpha \beta^{j}\right\}\text{ for $j \geq 1$.}
\end{align*}
In order for this partition to be legitimate, we need to establish that $\beta \geq 1$ and that the sets $\{S_j\}$ actually include all elements of $V^2$.
We will show now that $\beta$ is bounded on both sides by absolute constants.
\begin{lemma}\label{2xor_betasmall}
	\[1 \leq \beta = O(1).\]
\end{lemma}
\begin{proof}
	We first establish the upper bound.
	Since each of the $n$ elements of $V$ is in at most $d$ pairs in each of the $\ell$ partitions, we know $m \leq \ell d n = O(\poly(n))$.
	Then expanding $R$, $\alpha$, and $\beta$ we have
	\[\beta =
	\left(\frac{16\varepsilon^4 m^2}{Cd^2\ell\log(n)^6}\right)^{1/\log n} \leq O\left( \ell n^2\right)^{1/\log n}=
	O(\poly(n))^{1/\log n} = O(1).\]

	Next we establish the lower bound of 1.
	\[
	\beta =
	\left(\frac{16\varepsilon^4 m^2}{Cd^2\ell\log(n)^6}\right)^{1/\log n}
	\geq \left(\frac{\varepsilon^2 m}{Cd^2\log(n)^6}\right)^{1/\log n} \geq 1^{1/\log n} = 1.
	\]
	where the first inequality holds since we assumed $\ell \leq \varepsilon^2 m$ via our lower bound on $m$, and the second inequality holds since $d = O(\poly(\varepsilon^{-1}, \log n))$.
\end{proof}

By Lemma~\ref{2xor_gammasum} and nonnegativity of $\gamma$, we know $\gamma(v,v') \leq 4m = \alpha\beta^{\log n}$ always, so the $S_j$ do indeed cover all possible cases for $\gamma(v, v')$ and thus form a partition.

\begin{lemma}\label{2xor_sisize}
	$|S_0| \leq n^2$, and for $j \geq 1$,
	\[|S_j| \leq \frac{4m}{\alpha \beta^{j-1}}.\]
\end{lemma}
\begin{proof}
	The first bound follows as $S_0 \subseteq V^2$.
	For the second bound see that
	\[|S_j|\alpha \beta^{j-1} \leq \sum_{(v,v') \in S_j} \gamma(v,v') \leq \sum_{v,v' \in [n]} \gamma(v,v') \leq 4m\]
	where the last inequality follows from Lemma~\ref{2xor_gammasum}.
\end{proof}

The main idea of our refutation is as follows. A pair $(v,v')$ of high weight will bump up the value of $\Phi_1$.
However, Lemma~\ref{2xor_sisize} shows that there cannot be too many pairs contributing too large of a value.
To make this more precise, we will break $\Phi_1$ down even further into a sum of $(1 + \log n)^2$ different functions $\Phi_{j,k}$ indexed by $0 \leq j,k \leq \log n$.
The function $\Phi_{j,k}$ will be associated to the pair $(S_j, S_k)$.
We will then bound each of these $\Phi_{j,k}$ functions individually.
Let
\begin{equation*}
\Phi_{j,k}(x) = \sum_{i = 1}^\ell \frac{1}{\sqrt{t_i}} \sum_{\substack{u,u',v,v' \\ (u,v) \neq (u',v') \\ (v,v') \in S_j, (u,u') \in S_k}} x_v x_{u} x_{v'} x_{u'} r_i(v,u) r_i(v',u').
\end{equation*}

When taking $\sum_{j,k} \Phi_{j,k}(x)$ the conditions on the third line of the inner summation disappear, so $\sum_{j,k} \Phi_{j,k}(x) = \Phi_1(x)$.

Certifying that $\Phi_{j,k}(x)$ is small will take the form of an eigenvalue bound on a certain matrix.
Define the matrix $M$ by
\begin{align*}
	M(v,v';u,u') =
	\begin{cases}
	\sum_{i=1}^\ell \frac{1}{\sqrt{t_i}}r_i(v,u)r_i(v',u') &\text{when $(v,u) \neq (v',u')$, and} \\
	0 &\text{otherwise.}
	\end{cases}
\end{align*}
Let $x^{\otimes 2}$ be the vector with $(x^{\otimes 2})_{u,v} = x_u x_v$.
By tracing definitions, we see that
\begin{equation*}
(x^{\otimes 2})^\top M (x^{\otimes 2}) = \Phi_2(x).
\end{equation*}
The functions $\Phi_{j,k}$ correspond to the contribution of the submatrix of $M$ with rows in $S_j$ and columns in $S_k$.
More concretely, for each $0 \leq j,k \leq \log n$ let $M_{j,k}$ be the restriction of $M$ to rows indexed by $S_j$ and columns indexed by $S_k$.
Let $x^{\otimes 2}_{|S_i}$ be the restriction of $X^{\otimes 2}$ to indices in $S_i$.
Then
\[(x^{\otimes 2}_{|S_j})^{\top} M_{j,k} (x^{\otimes 2}_{|S_k}) = \Phi_{j,k}(x)\]
So it suffices to bound this quantity.
Since $x^{\otimes 2}_{|S_j} \in \{\pm 1\}^{S_j}$, we have
\begin{equation}
\Phi_{j,k}(x) = (x^{\otimes 2}_{|S_j})^{\top} M_{j,k} (x^{\otimes 2}_{|S_k}) \leq \sqrt{|S_j| \cdot |S_k|} \cdot \|M_{j,k}\|.
\end{equation}
We already have upper bounds on the sizes of $S_j$ and $S_k$, so what remains is to show that $\|M_{j,k}\|$ is small with high probability.

\begin{lemma}\label{2xor_mnormsmall}
	For all $0 \leq j,k \leq \log n$, we have
	\[\|M_{j,k}\| = O\left(d\sqrt{\alpha \beta^{\max(j,k)}} \log(n)\right).\]
	with high probability.
\end{lemma}

The key ingredient in the proof of Lemma~\ref{2xor_mnormsmall} is the rectangular matrix Bernstein inequality, stated earlier as Theorem~\ref{mbernstein_rect}.
To apply it, we will write $M_{j,k}$ as a sum of independent, zero-mean matrices $B_{i,j,k}$ for $1 \leq i \leq \ell$, and provide upper bounds on both $\|B_{i,j,k}\|$ and the variance term $\sigma^2$ from the statement of the matrix Bernstein inequality.
We begin by defining the matrix $B_{i,j,k} \in \mathbb{R}^{S_j \times S_k}$ as
\begin{equation}
	B_{i,j,k}(v,v';u,u') =
	\begin{cases} \frac{1}{\sqrt{t_i}}r_i(v,u)r_i(v',u') &\text{when $(v,u) \neq (v',u')$, and} \\
	0 &\text{otherwise.}
	\end{cases}
\end{equation}
It follows from definitions that $\sum_{i=1}^\ell B_{i,j,k} = M_{j,k}$.
The following lemma shows that $d$-bounded property implies that $B_{i,j,k}$ is $d^2$-sparse in each row and column.
\begin{lemma}\label{2xor_bsparse}
	For all $0 \leq j,k \leq \log n$ and $1 \leq i \leq n$, the matrix $B_{i,j,k}$ has at most $d^2$ entries in every row and column.
\end{lemma}
\begin{proof}
	We prove the lemma for rows, and the case for columns follows analogously.
	Consider an arbitrary row $(v,v')$ of $B_{i,j,k}$.
	For any $v \in V$, let $S(v)$ be the set of $u \in V$ such that $(u,v) \in T_i$.
	Since each $v$ appears in at most $d$ different pairs in $T_i$, we know $|S(v)| \leq d$ for all $v \in V$.
	Let $W = \{(u,u') \mid B_{i,j,k}(v,v';u,u') \neq 0\}$ be the set of nonzero columns in the row $B_{i,j,k}(v,v';-,-)$.
	If $(u,u') \in W$ then $B_{i,j,k}(v,v';u,u') \neq 0$, meaning $(v,u),(v',u') \in T_i$ so $(u,u') \in S(v) \times S(v')$.
	Therefore $|W| \leq |S(v) \times S(v')| \leq d^2$.
\end{proof}
We now establish a uniform bound on the spectral norm of $B_{i,j,k}$.
\begin{lemma}\label{2xor_bibound}
	For all $0 \leq j,k \leq \log n$ and $1 \leq i \leq n$,
	\[\|B_{i,j,k}\| \leq d \sqrt{\alpha \beta^{\max(j,k)}}\]
\end{lemma}
\begin{proof}
	Let $z(v,v')$ be the row vector corresponding to row $(v,v')$ in $B_{i,j,k}$.
	We first bound $\|z(v,v')\|_2$ by seeing that 
	\begin{align*}
		\|z(v,v')\|_2^2
		&= \sum_{(u,u') \in S_k} B_{i,j,k}(v,v';u,u')^2 \\
		&= \sum_{\substack{(u,u') \in S_k \\ (v,u) \neq (v',u')}} \frac{r_i(v,u)^2r_i(v',u')^2}{t_i} \\
		&= \frac{\deg_i(v)\deg_i(v')}{t_i} \\
		&\leq \gamma(v,v').
	\end{align*}
	So $\|z(v,v')\|_2 \leq \sqrt{\gamma(v,v')} \leq \sqrt{\alpha \beta^j}$, where the second inquality follows since $(v,v') \in S_j$.
	Since $z(u,u')$ is $d^2$-sparse, we have $\|z(v,v')\|_1 \leq d\|z(v,v')\|_2 \leq d\sqrt{\alpha b^j}$.
	Thus the maximum $\ell_1$ norm of any row in $B_{i,j,k}$ is at most $d\sqrt{\alpha \beta^j}$.

	An analogous argument shows that the maximum $\ell_1$ norm of any column in $B_{i,j,k}$ is at most $d\sqrt{\alpha \beta^k}$.
	Combined with Lemma~\ref{gersh_rect}, this completes the proof.
\end{proof}

All that remains is to bound the variance term in the statement of Theorem~\ref{mbernstein_rect}.
We prove the following lemma.
\begin{lemma}\label{2xor_variancebound}
	For $0 \leq j, k \leq \log n$, we have
	\[\max\left\{\left\|\sum_{i=1}^\ell \E[B_{i,j,k} B_{i,j,k}^\top]\right\|,\left\|\sum_{i=1}^\ell \E[B_{i,j,k}^\top B_{i,j,k}]\right\| \right\}\leq 2\alpha \beta^{\max(j,k)}\]
\end{lemma}

\begin{proof}
	Let $X_{j,k} = \sum_{i=1}^\ell \E[B_{i,j,k}B_{i,j,k}^\top]$.
	Because $B_{i,j,k} = B_{i,k,j}^\top$, the value we would like to bound is $\max\{\|X_{j,k}\|,\|X_{k,j}\|\}$.
	Then it suffices to show that $\|X_{j,k}\| \leq 2\alpha \beta^j$.

	We will first show that $X_{j,k}(v,v';u,u') \neq 0$ implies $\{v,v'\} = \{u, u'\}$.
	We expand the definition to find
	\begin{align*}
		X_{j,k}(v,v';u,u')
		&= \sum_{i = 1}^\ell\sum_{w,w'} \E[B_{i,j,k}(v,v';w,w')B_{i,j,k}(u,u';w,w')] \\
		&= \sum_{i = 1}^\ell \frac{1}{t_i} \sum_{\substack{(w,w') \in S_k \\ (v,w) \neq (v',w') \\ (u,w) \neq (u',w')}}\E[r_i(v,w)r_i(v',w')r_i(u,w)r_i(u',w')]
	\end{align*}
	For any $e,e' \in T_i$ either $r_i(e)$ and $r_i(e')$ are identical or $r_i(e)$ and $r_i(e')$ are independent with zero-mean, so each term inside the expectation is either 0 or 1.
	This tells us that $X_{j,k}$ is a nonnegative matrix.
	A term is equal to 1 precisely when the four $r(-)$ factors can be partitioned into two equal pairs.
	We cannot pair factors 1 and 2 since $\{v,w\} \neq \{v',w'\}$ by the condition on indices we are summing over.

	Suppose factors 1 and 3 are equal, and additionally factors 2 and 4 are equal. 
	Then we can see directly that $v = u$ and $v' = u'$.

	Suppose factors 1 and 4 are equal, and additionally factors 2 and 3 are equal.
	Then either (1) $v = u'$ and $w = w'$, or (2) $v = w'$ and $w = u'$.
	By looking at factors 2 and 3, case (1) implies $v' = u$, meaning $(v,v') = (u',u)$.
	Again looking at factors 2 and 3, case (2) implies $\{v,v'\} = \{u,u'\}$.

	Thus by considering all cases, we have determined that $X_{j,k}(v,v';u,u')$ is only ever nonzero when $\{v,v'\} = \{u,u'\}$.
	In the case $v = u$ and $v' = u'$, we see
	\begin{align*}
	X_{j,k}(v,v';v,v')
	&= \sum_{i=1}^\ell \frac{1}{t_i} \sum_{\substack{(w,w') \in S_j \\ (v,w) \neq (v',w')}} r_i(v,w)^2 r_i(v',w')^2 \\
	&\leq \sum_{i=1}^\ell \frac{\deg_i(v) \deg_i(v')}{t_i} \\
	&= \gamma(v,v') \leq \alpha \beta^j
	\end{align*}
	where the last inequality follows since $(v,v') \in S_j$.
	When $v = u'$ and $v' = u$, we see
	\begin{align*}
		X_{j,k}(v,v';v',v)
		&= \sum_{i = 1}^\ell \frac{1}{t_i} \sum_{\substack{(w,w') \in S_k \\ (v,w) \neq (v',w') \\ (v',w) \neq (v,w')}}\E[r_i(v,w)r_i(v',w')r_i(v',w)r_i(v,w')] \\
		&\leq \sum_{i = 1}^\ell \frac{1}{t_i} \sum_{(w,w') \in V}r_i(v,w)^2r_i(v',w')^2 \\
		&= \gamma(v,v') \leq \alpha \beta^j
	\end{align*}
	where the last equality is because $(v,v'),(v',v) \in S_j$.
	Then each row and column of $X_{j,k}$ has at most two nonzero entries, each bounded by $\gamma(v,v') \leq \alpha \beta^j$.
	Then Lemma~\ref{gersh_rect} applies to show $\|X_{j,k}\| \leq 2\alpha \beta^j$, completing the proof.
\end{proof}

We now have enough information to apply the matrix Bernstein inequality to the decomposition $M_{j,k} = \sum_{i=1}^\ell B_{i,j,k}$.
By Theorem~\ref{mbernstein_rect}, Lemma~\ref{2xor_bibound}, and Lemma~\ref{2xor_variancebound}, we can set some $t = O\left(d \sqrt{\alpha \beta^{\max(i,j)}} \log(n)\right)$ so that 
\begin{align*}
	\operatorname{P}\left[\|M_{j,k}\| \geq t\right]
	&\leq (|S_j| + |S_k|)\exp\left(\frac{-t^2/2}{2\alpha \beta^{\max(j,k)}+d\sqrt{\alpha \beta^{\max(j,k)}} t/3}\right) \\
	&\leq n2^{-O(\log n)} \\
	& \leq \frac{1}{p(n)}
\end{align*}
for an arbitrarily high degree polynomial $p$.
This completes the proof of Lemma~\ref{2xor_mnormsmall}.
Since there are only $(1+\log n)^2$ different $M_{j,k}$ the probability that $\|M_{j,k}\| = O(\alpha \beta^{\max(i,j)})$ for all of them is at least $1-\frac{1}{p(n)}$ for a polynomial $p$ of arbitrarily high degree.
We now show that in the highly probable case that this bound holds for all $M_{j,k}$, $\Phi_2(x) \leq \frac{\varepsilon^2 m^{3/2}}{\sqrt{\ell}}$ for all $x \in \{\pm 1\}^n$.

Note that we have the inequality
\begin{equation} \label{phi2_max_bound}
\Phi_2(x) = \sum_{0 \leq j,k \leq \log n} \Phi_{j,k}(x) \leq \log(n)^2 O\left(\max_{0 \leq j,k \leq \log n} \Phi_{j,k}(x)\right)
\end{equation}

Since our upper bound on $|S_j|$ from Lemma~\ref{2xor_sisize} depends on whether $j = 0$ or not, we break into three cases when bounding all $\Phi_{j,k}(x)$.
We only consider the case when $j \leq k$, since $\Phi_{j,k}(x) = \Phi_{k,j}(x)$.

When $j = k = 0$, we have
\begin{align*}
\Phi_{0,0}(x)
&\leq \sqrt{|S_0| \cdot |S_0|}\|M_{0,0}\| \\
&\leq n^2\|M_{0,0}\| \tag{by Lemma~\ref{2xor_sisize}} \\
&= O\left(dn^2\sqrt{\alpha}\log(n)\right) \tag{by Lemma~\ref{2xor_mnormsmall}} \\
&= O\left(\frac{d\sqrt{R\ell} n^2 \log(n)}{\sqrt{m}}\right)
\end{align*}

When $j = 0$ and $k \geq 1$ we have
\begin{align*}
\Phi_{0,k}(x)
&\leq \sqrt{|S_0| \cdot |S_k|}\|M_{0,k}\| \\
&\leq n\sqrt{\frac{4m}{\alpha \beta^{k-1}}}\|M_{0,k}\| \tag{by Lemma~\ref{2xor_sisize}} \\
&= O\left(n\sqrt{\beta} d\sqrt{m}\log(n)\right) \tag{by Lemma~\ref{2xor_mnormsmall}} \\
&= O\left(dn\sqrt{m}\log(n)\right) \tag{by Lemma~\ref{2xor_betasmall}}
\end{align*}

and when $1 \leq j \leq k$ we have
\begin{align*}
\Phi_{j,k}(x)
&\leq \sqrt{|S_j| \cdot |S_k|}\|M_{j,k}\| \\
&\leq \frac{4m}{\alpha \beta^{(j+k-2)/2}} \|M_{j,k}\| \tag{by Lemma~\ref{2xor_sisize}}\\
&= O\left(\frac{dm\log(n)}{\sqrt{\alpha}\beta^{(j-2)/2}}\right) \tag{by Lemma~\ref{2xor_mnormsmall}}\\
&= O\left(\frac{dm^{3/2}\log(n)}{\sqrt{R\ell}}\right) \tag{by Lemma~\ref{2xor_betasmall}}\\
\end{align*}

Recall that we defined $R = \frac{Cd^2 \log^6 n}{\varepsilon^4}$ for some large enough absolute constant $C$.
It is straightforward to verify that all three of the above bounds can be made less than any fixed constant fraction of $\frac{\varepsilon^2 m^{3/2}}{\sqrt{\ell}\log(n)^2}$ by adjusting the constant $C$ in the definition of $R$, and the constant $K$ in the lower bound on $m$ from the statement of Theorem~\ref{2xor_bounded_partitioned}.
We then apply Inequality~(\ref{phi2_max_bound}) to see
\[\Phi_2(x) \leq \log(n)^2 O\left(\max_{j,k} \Phi_{j,k}(x)\right) \leq \frac{\varepsilon^2 m^{3/2}}{\sqrt{\ell}}.\]
This completes the proof of Theorem~\ref{2xor_bounded_partitioned}.

==> preamble/macros-custom.tex <==
% algorithm packages


%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{algpseudocode}

%\algnewcommand\algorithmicinput{\textbf{Input:}}
%\algnewcommand\INPUT{\item[\algorithmicinput]}
%\algnewcommand\algorithmicoutput{\textbf{Output:}}
%\algnewcommand\OUTPUT{\item[\algorithmicoutput]}

% paper-specific packages
\usepackage{relsize}
\usepackage[font=footnotesize]{caption}
\usepackage{appendix}


% abbreviations and paper-specific macros

% math
\newcommand{\D}{\mathcal{D}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\on}{\{-1,1\}}
\newcommand{\sphere}{\bbS^{n-1}}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\lamax}{\lambda_{\mathrm{max}}}
\newcommand{\Sn}{\mathbb{S}^{n-1}}
\DeclareMathOperator{\Id}{\mathrm{Id}}
\DeclareMathOperator{\F}{\mathbb{F}}
\DeclareMathOperator{\codim}{codim}


% not math
\DeclareUrlCommand\email{}
\newcommand{\whp}{\text{w.h.p.}}
\newcommand{\wovp}{\text{w.ov.p.}\xspace}
\newcommand{\YES}{\textsc{yes}\xspace}
\newcommand{\NO}{\textsc{no}\xspace}

\newcommand{\wovple}{\hspace{-3mm}\stackrel{\text{\wovp}}{\le}}
\newcommand{\wovpeq}{\hspace{-3mm}\stackrel{\text{\wovp}}{=}}
\newcommand{\wovpge}{\hspace{-3mm}\stackrel{\text{\wovp}}{\ge}}
\newcommand{\aasle}{\hspace{-1.5mm}\stackrel{\text{a.a.s.}}\le}

\newcommand{\Pisymm}{\Pi_{\mathrm{symm}}}
\newcommand{\Pisym}{\Pi_{\mathrm{sym}}}

%added by TM
\newcommand{\inner}[1]{\langle #1 \rangle}
\newcommand{\sosle}{\preceq}
\newcommand{\sosge}{\succeq}

\DeclareMathOperator{\tE}{\tilde{\mathbb E}}
\DeclareMathOperator{\tO}{\tilde{O}}
\newcommand{\ta}{\tilde{a}}
\newcommand{\tA}{\tilde{A}}


\DeclareMathOperator*{\pE}{\tilde{\mathbb E}}

\newcommand{\bT}{\mathbf{T}}
\newcommand{\ot}{\otimes}
\newcommand{\tr}{\textup{tr}}
\newcommand{\diag}{\textup{diag}}

\let\pref=\prettyref

% transpose
% http://tex.stackexchange.com/questions/204892/visually-appealing-subscripts-with-intercal
% http://tex.stackexchange.com/questions/30619/what-is-the-best-symbol-for-vector-matrix-transpose
\newcommand*{\transpose}[1]{{#1}{}^{\mkern-4mu\intercal}}
\newcommand*{\vardyad}[1]{#1^{\vphantom{\intercal}}#1^{\intercal}}
\newcommand*{\dyad}[1]{#1#1{}^{\mkern-4mu\intercal}}

% \let\Id\undefined
% \newcommand*{\Id}{I}

% span of subspace -- temporary

\newcommand{\sspan}{\textup{span}}
\newcommand{\1}{\bm{1}}

\newcommand{\Cov}{\mathop{\mathrm{Cov}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../planted"
%%% End:


==> preamble/macros.tex <==
% {{{ etex }}}

\usepackage{etex}

% {{{ nag }}}

\usepackage[l2tabu, orthodox]{nag}

% {{{ common }}}

\usepackage{xspace,enumerate}

\usepackage[dvipsnames]{xcolor}

\usepackage[T1]{fontenc}
\usepackage[full]{textcomp}

% {{{ babelamerican }}}
\usepackage[american]{babel}

% {{{ mathtools }}}

\usepackage{mathtools}


% {{{ boldmath }}}

% fix for "too many math alphabets" problem
\newcommand\hmmax{0} % default 3
% \usepackage{bm}

% \usepackage{stmaryrd}


% {{{ amsthm }}}
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}

\newtheorem{subclaim}{Claim}[theorem]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheorem*{fact*}{Fact}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem*{hypothesis*}{Hypothesis}
\newtheorem{conjecture}[theorem]{Conjecture}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{protocol}[theorem]{Protocol}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{observation}[theorem]{Observation}
\newtheorem*{observation*}{Observation}



% {{{ geometry-nice }}}


\ifnum\writemode=1
\usepackage[
letterpaper,
top=1.2in,
bottom=1.2in,
left=1in,
right=1in]{geometry}

\pagestyle{empty}
\fi

\ifnum\writemode=0
\usepackage[
letterpaper,
top=0.7in,
bottom=0.9in,
left=1in,
right=1in]{geometry}
\fi

% {{{ fonts }}}

\usepackage{newpxtext} % T1, lining figures in math, osf in text
\usepackage{textcomp} % required for special glyphs
\usepackage[varg,bigdelims]{newpxmath}
\usepackage[scr=rsfso]{mathalfa}% \mathscr is fancier than \mathcal
\usepackage{bm} % load after all math to give access to bold math
% \useosf %no longer needed
\linespread{1.1}% Give Palatino more leading (space between lines)
\let\mathbb\varmathbb

% {{{ showkeys }}}

\ifnum\showkeys=1
\usepackage[color]{showkeys}
\fi

% {{{ hyperref-option2 }}}

\ifnum\showcolorlinks=1
\usepackage[
pagebackref,
% letterpaper=true,
colorlinks=true,
urlcolor=blue,
linkcolor=blue,
citecolor=OliveGreen,
]{hyperref}
\fi

\ifnum\showcolorlinks=0
\usepackage[
pagebackref,
% letterpaper=true,
colorlinks=false,
pdfborder={0 0 0}
]{hyperref}
\fi


\usepackage[capitalise,nameinlink]{cleveref}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{definition}{Definition}{Definitions}

% {{{ prettyref }}}

% \usepackage{prettyref}

% % From manual:
% % \newrefformat{eq}{\textup{(\ref{#1})}}
% % \newrefformat{lem}{Lemma~\ref{#1}}
% % \newrefformat{thm}{Theorem~\ref{#1}}
% % \newrefformat{cha}{Chapter~\ref{#1}}
% % \newrefformat{sec}{Section~\ref{#1}}
% % \newrefformat{tab}{Table~\ref{#1} on page~\pageref{#1}}
% % \newrefformat{fig}{Figure~\ref{#1} on page~\pageref{#1}}

% \newcommand{\savehyperref}[2]{\texorpdfstring{\hyperref[#1]{#2}}{#2}}

% \newrefformat{eq}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
% \newrefformat{eqn}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
% \newrefformat{lem}{\savehyperref{#1}{Lemma~\ref*{#1}}}
% \newrefformat{def}{\savehyperref{#1}{Definition~\ref*{#1}}}
% \newrefformat{thm}{\savehyperref{#1}{Theorem~\ref*{#1}}}
% \newrefformat{cor}{\savehyperref{#1}{Corollary~\ref*{#1}}}
% \newrefformat{cha}{\savehyperref{#1}{Chapter~\ref*{#1}}}
% \newrefformat{sec}{\savehyperref{#1}{Section~\ref*{#1}}}
% \newrefformat{app}{\savehyperref{#1}{Appendix~\ref*{#1}}}
% \newrefformat{tab}{\savehyperref{#1}{Table~\ref*{#1}}}
% \newrefformat{fig}{\savehyperref{#1}{Figure~\ref*{#1}}}
% \newrefformat{hyp}{\savehyperref{#1}{Hypothesis~\ref*{#1}}}
% \newrefformat{alg}{\savehyperref{#1}{Algorithm~\ref*{#1}}}
% \newrefformat{rem}{\savehyperref{#1}{Remark~\ref*{#1}}}
% \newrefformat{item}{\savehyperref{#1}{Item~\ref*{#1}}}
% \newrefformat{step}{\savehyperref{#1}{step~\ref*{#1}}}
% \newrefformat{conj}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
% \newrefformat{fact}{\savehyperref{#1}{Fact~\ref*{#1}}}
% \newrefformat{prop}{\savehyperref{#1}{Proposition~\ref*{#1}}}
% \newrefformat{prob}{\savehyperref{#1}{Problem~\ref*{#1}}}
% \newrefformat{claim}{\savehyperref{#1}{Claim~\ref*{#1}}}
% \newrefformat{relax}{\savehyperref{#1}{Relaxation~\ref*{#1}}}
% \newrefformat{red}{\savehyperref{#1}{Reduction~\ref*{#1}}}
% \newrefformat{part}{\savehyperref{#1}{Part~\ref*{#1}}}



% {{{ sref }}}

% short section reference
\newcommand{\Sref}[1]{\hyperref[#1]{\S\ref*{#1}}}

% {{{ nicefrac }}}
% commands for fractions
\usepackage{nicefrac}
% poor man's fraction
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\varflatfrac}[2]{#1\textfractionsolidus#2}

\let\nfrac=\nicefrac
\let\ffrac=\flatfrac
% similar commands: tfrac,dfrac

\newcommand{\half}{\nicefrac12}
\newcommand{\onequarter}{\nicefrac14}
\newcommand{\threequarter}{\nicefrac34}

% {{{ microtype-option }}}

\ifnum\usemicrotype=1
\usepackage{microtype}
\fi

% {{{ authornotes }}}
\ifnum\showauthornotes=1
\newcommand{\Authornote}[2]{{\sffamily\small\color{red}{[#1: #2]}}}
\newcommand{\Authornotecolored}[3]{{\sffamily\small\color{#1}{[#2: #3]}}}
\newcommand{\Authorcomment}[2]{{\sffamily\small\color{gray}{[#1: #2]}}}
\newcommand{\Authorstartcomment}[1]{\sffamily\small\color{gray}[#1: }
\newcommand{\Authorendcomment}{]\rmfamily\normalsize\color{black}}
\newcommand{\Authorfnote}[2]{\footnote{\color{red}{#1: #2}}}
\newcommand{\Authorfixme}[1]{\Authornote{#1}{\textbf{??}}}
\newcommand{\Authormarginmark}[1]{\marginpar{\textcolor{red}{\fbox{\Large #1:!}}}}
\else
\newcommand{\Authornote}[2]{}
\newcommand{\Authornotecolored}[3]{}
\newcommand{\Authorcomment}[2]{}
\newcommand{\Authorstartcomment}[1]{}
\newcommand{\Authorendcomment}{}
\newcommand{\Authorfnote}[2]{}
\newcommand{\Authorfixme}[1]{}
\newcommand{\Authormarginmark}[1]{}
\fi

\newcommand{\Dnote}{\Authornote{D}}
%\newcommand{\Tnote}{\Authornotecolored{blue}{T}}
\newcommand{\TMnote}{\Authornotecolored{blue}{T}}
\newcommand{\Inote}{\Authornotecolored{ForestGreen}{I}}
\newcommand{\inote}{\Inote}
\newcommand{\Gnote}{\Authornote{G}}
\newcommand{\Jcomment}{\Authorcomment{J}}
\newcommand{\Dcomment}{\Authorcomment{D}}
\newcommand{\Dstartcomment}{\Authorstartcomment{D}}
\newcommand{\Dendcomment}{\Authorendcomment}
\newcommand{\Dfixme}{\Authorfixme{D}}
\newcommand{\Dmarginmark}{\Authormarginmark{D}}
\newcommand{\Dfnote}{\Authorfnote{D}}

\newcommand{\Pnote}{\Authornote{P}}
\newcommand{\Pfnote}{\Authorfnote{P}}

\newcommand{\PRnote}{\Authornote{PR}}
\newcommand{\PRfnote}{\Authorfnote{PR}}

\newcommand{\PTnote}{\Authornote{PT}}
\newcommand{\PTfnote}{\Authorfnote{PT}}

\newcommand{\PGnote}{\Authornote{PG}}
\newcommand{\PGfnote}{\Authorfnote{PG}}

\newcommand{\Bnote}{\Authornote{B}}
\newcommand{\Bfnote}{\Authorfnote{B}}

\definecolor{forestgreen(traditional)}{rgb}{0.0, 0.27, 0.13}
\newcommand{\Jnote}{\Authornotecolored{forestgreen(traditional)}{J}}
\newcommand{\Jfnote}{\Authorfnote{J}}


\newcommand{\Mnote}{\Authornote{M}}
\newcommand{\Mfnote}{\Authorfnote{M}}

\newcommand{\Rnote}{\Authornote{M}}
\newcommand{\Rfnote}{\Authorfnote{M}}

\newcommand{\Nnote}{\Authornote{N}}
\newcommand{\Nfnote}{\Authorfnote{N}}

\newcommand{\Snote}{\Authornote{S}}
\newcommand{\Sfnote}{\Authorfnote{S}}


% {{{ fixme }}}

% place red exclamation mark in margin
%\newcommand{\redmarginmarker}{\marginpar{\textcolor{red}{\fbox{\Large !}}}}
\newcommand{\redmarginmarker}{}

% short indicator for places that need fixing
\newcommand{\FIXME}{\textbf{\textcolor{red}{??}}\redmarginmarker}

\ifnum\showfixme=0
\renewcommand{\FIXME}{}
\fi


% {{{ boxedminipage }}}
\usepackage{boxedminipage}

\newenvironment{mybox}
{\center \noindent\begin{boxedminipage}{1.0\linewidth}}
{\end{boxedminipage}
\noindent
}


% {{{ parentheses }}}
% various bracket-like commands
% round parentheses
\newcommand{\paren}[1]{(#1)}
\newcommand{\Paren}[1]{\left(#1\right)}
\newcommand{\bigparen}[1]{\big(#1\big)}
\newcommand{\Bigparen}[1]{\Big(#1\Big)}
% square brackets
\newcommand{\brac}[1]{[#1]}
\newcommand{\Brac}[1]{\left[#1\right]}
\newcommand{\bigbrac}[1]{\big[#1\big]}
\newcommand{\Bigbrac}[1]{\Big[#1\Big]}
\newcommand{\Biggbrac}[1]{\Bigg[#1\Bigg]}
% absolute value
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigabs}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigabs}[1]{\Big\lvert#1\Big\rvert}
% cardinality
\newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\Card}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigcard}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigcard}[1]{\Big\lvert#1\Big\rvert}
% set
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\bigset}[1]{\big\{#1\big\}}
\newcommand{\Bigset}[1]{\Big\{#1\Big\}}
% norm
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bignorm}[1]{\big\lVert#1\big\rVert}
\newcommand{\Bignorm}[1]{\Big\lVert#1\Big\rVert}
\newcommand{\Biggnorm}[1]{\Bigg\lVert#1\Bigg\rVert}
% 2-norm
\newcommand{\normt}[1]{\norm{#1}_2}
\newcommand{\Normt}[1]{\Norm{#1}_2}
\newcommand{\bignormt}[1]{\bignorm{#1}_2}
\newcommand{\Bignormt}[1]{\Bignorm{#1}_2}
% 2-norm squared
\newcommand{\snormt}[1]{\norm{#1}^2_2}
\newcommand{\Snormt}[1]{\Norm{#1}^2_2}
\newcommand{\bigsnormt}[1]{\bignorm{#1}^2_2}
\newcommand{\Bigsnormt}[1]{\Bignorm{#1}^2_2}
% norm squared
\newcommand{\snorm}[1]{\norm{#1}^2}
\newcommand{\Snorm}[1]{\Norm{#1}^2}
\newcommand{\bigsnorm}[1]{\bignorm{#1}^2}
\newcommand{\Bigsnorm}[1]{\Bignorm{#1}^2}
% 1-norm
\newcommand{\normo}[1]{\norm{#1}_1}
\newcommand{\Normo}[1]{\Norm{#1}_1}
\newcommand{\bignormo}[1]{\bignorm{#1}_1}
\newcommand{\Bignormo}[1]{\Bignorm{#1}_1}
% infty-norm
\newcommand{\normi}[1]{\norm{#1}_\infty}
\newcommand{\Normi}[1]{\Norm{#1}_\infty}
\newcommand{\bignormi}[1]{\bignorm{#1}_\infty}
\newcommand{\Bignormi}[1]{\Bignorm{#1}_\infty}
% inner product
\newcommand{\iprod}[1]{\langle#1\rangle}
\newcommand{\Iprod}[1]{\left\langle#1\right\rangle}
\newcommand{\bigiprod}[1]{\big\langle#1\big\rangle}
\newcommand{\Bigiprod}[1]{\Big\langle#1\Big\rangle}


% {{{ probability }}}
% expectation, probability, variance
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}

\DeclareMathOperator*{\E}{\Esymb}
\DeclareMathOperator*{\Var}{\Vsymb}
\DeclareMathOperator*{\ProbOp}{\Psymb}

\renewcommand{\Pr}{\ProbOp}

% TODO: make case distinction if optional argument is not set
\newcommand{\prob}[1]{\Pr\set{#1}}
\newcommand{\Prob}[2][]{\Pr_{{#1}}\Set{#2}}

\newcommand{\ex}[1]{\E\brac{#1}}
\newcommand{\Ex}[2][]{\E_{{#1}}\Brac{#2}}
\newcommand{\varex}[1]{\E\paren{#1}}
\newcommand{\varEx}[1]{\E\Paren{#1}}

%\newcommand{\given}{\;\middle\vert\;}
\newcommand{\given}{\mathrel{}\middle\vert\mathrel{}}
%\newcommand{\given}{\mathrel{}\middle|\mathrel{}}

% {{{ mathfonts }}}

% \usepackage{dsfont}
% \usepackage{yfonts}
% \usepackage{mathrsfs}


% {{{ miscmacros }}}

% middle delimiter in the definition of a set
\newcommand{\suchthat}{\;\middle\vert\;}

% tensor product
\newcommand{\tensor}{\otimes}

% add explanations to math displays
\newcommand{\where}{\text{where}}
\newcommand{\textparen}[1]{\text{(#1)}}
\newcommand{\using}[1]{\textparen{using #1}}
\newcommand{\smallusing}[1]{\text{(\small using #1)}}
\ifx\because\undefined
\newcommand{\because}[1]{\textparen{because #1}}
\else
\renewcommand{\because}[1]{\textparen{because #1}}
\fi
\newcommand{\by}[1]{\textparen{by #1}}


% spectral order (Loewner order)
\newcommand{\sge}{\succeq}
\newcommand{\sle}{\preceq}

% smallest and largest eigenvalue
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\lmax}{\lambda_{\max}}

\newcommand{\signs}{\set{1,-1}}
\newcommand{\varsigns}{\set{\pm 1}}
\newcommand{\maximize}{\mathop{\textrm{maximize}}}
\newcommand{\minimize}{\mathop{\textrm{minimize}}}
\newcommand{\subjectto}{\mathop{\textrm{subject to}}}

\renewcommand{\ij}{{ij}}

% symmetric difference
\newcommand{\symdiff}{\Delta}
\newcommand{\varsymdiff}{\bigtriangleup}

% set of bits
\newcommand{\bits}{\{0,1\}}
\newcommand{\sbits}{\{\pm1\}}

% no stupid bullets for itemize environmentx
% \renewcommand{\labelitemi}{--}

% control white space of list and display environments
\newcommand{\listoptions}{\labelsep0mm\topsep-0mm\itemindent-6mm\itemsep0mm}
\newcommand{\displayoptions}[1]{\abovedisplayshortskip#1mm\belowdisplayshortskip#1mm\abovedisplayskip#1mm\belowdisplayskip#1mm}

% short for emptyset
%\newcommand{\eset}{\emptyset}
% moved to mathabbreviations

% short for epsilon
%\newcommand{\e}{\epsilon}
% moved to mathabbreviations

% super index with parentheses
\newcommand{\super}[2]{#1^{\paren{#2}}}
\newcommand{\varsuper}[2]{#1^{\scriptscriptstyle\paren{#2}}}

% tensor power notation
\newcommand{\tensorpower}[2]{#1^{\tensor #2}}


% multiplicative inverse
\newcommand{\inv}[1]{{#1^{-1}}}

% dual element
\newcommand{\dual}[1]{{#1^*}}

% subset
%\newcommand{\sse}{\subseteq}
% moved to mathabbreviations

% vertical space in math formula
\newcommand{\vbig}{\vphantom{\bigoplus}}

% setminus
\newcommand{\sm}{\setminus}

% define something by an equation (display)
\newcommand{\defeq}{\stackrel{\mathrm{def}}=}


% define something by an equation (inline)
\newcommand{\seteq}{\mathrel{\mathop:}=}



% declare function f by $f \from X \to Y$
\newcommand{\from}{\colon}

% big middle separator (for conditioning probability spaces)
\newcommand{\bigmid}{~\big|~}
\newcommand{\Bigmid}{~\Big|~}
\newcommand{\Mid}{\;\middle\vert\;}

% better vector definition and some variations
%\renewcommand{\vec}[1]{{\bm{#1}}}
\newcommand{\bvec}[1]{\bar{\vec{#1}}}
\newcommand{\pvec}[1]{\vec{#1}'}
\newcommand{\tvec}[1]{{\tilde{\vec{#1}}}}

% punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

% inner product for matrices
\newcommand\bdot\bullet

% transpose
\newcommand{\trsp}[1]{{#1}^\dagger}

% indicator function / vector
\ifx\mathds\undefined % use double stroke fonts if available
\DeclareMathOperator{\Ind}{\mathbb{I}}
\else
\DeclareMathOperator{\Ind}{\mathds 1}}
\fi

% place a qed symbol inside display formula
%\qedhere

% {{{ superscripts }}}

\renewcommand{\th}{\textsuperscript{th}\xspace}
\newcommand{\st}{\textsuperscript{st}\xspace}
\newcommand{\nd}{\textsuperscript{nd}\xspace}
\newcommand{\rd}{\textsuperscript{rd}\xspace}


% {{{ mathoperators }}}
\DeclareMathOperator{\Inf}{Inf}
\DeclareMathOperator{\Tr}{Tr}
%\newcommand{\Tr}{\mathrm{Tr}}
\DeclareMathOperator{\SDP}{SDP}
\DeclareMathOperator{\sdp}{sdp}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\opt}{opt}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\qpoly}{qpoly}
\DeclareMathOperator{\qpolylog}{qpolylog}
\DeclareMathOperator{\qqpoly}{qqpoly}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\Conv}{Conv}

\DeclareMathOperator{\rank}{rank}

% operators with limits
\DeclareMathOperator*{\median}{median}
\DeclareMathOperator*{\Median}{Median}

% smaller summation/product symbols
\DeclareMathOperator*{\varsum}{{\textstyle \sum}}
\DeclareMathOperator{\tsum}{{\textstyle \sum}}

\let\varprod\undefined

\DeclareMathOperator*{\varprod}{{\textstyle \prod}}
\DeclareMathOperator{\tprod}{{\textstyle \prod}}




% {{{ differentials }}}

\newcommand{\diffmacro}[1]{\,\mathrm{d}#1}

\newcommand{\dmu}{\diffmacro{\mu}}
\newcommand{\dgamma}{\diffmacro{\gamma}}
\newcommand{\dlambda}{\diffmacro{\lambda}}
\newcommand{\dx}{\diffmacro{x}}
\newcommand{\dt}{\diffmacro{t}}



% {{{ textabbreviations }}}

% some abbreviations
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\phd}{Ph.\,D.\xspace}
\newcommand{\msc}{M.\,S.\xspace}
\newcommand{\bsc}{B.\,S.\xspace}

\newcommand{\etal}{et al.\xspace}

\newcommand{\iid}{i.i.d.\xspace}

% {{{ foreignwords }}}

\newcommand\naive{na\"{\i}ve\xspace}
\newcommand\Naive{Na\"{\i}ve\xspace}
\newcommand\naively{na\"{\i}vely\xspace}
\newcommand\Naively{Na\"{\i}vely\xspace}




% {{{ names }}}
% Hungarian/Polish/East European names
\newcommand{\Erdos}{Erd\H{o}s\xspace}
\newcommand{\Renyi}{R\'enyi\xspace}
\newcommand{\Lovasz}{Lov\'asz\xspace}
\newcommand{\Juhasz}{Juh\'asz\xspace}
\newcommand{\Bollobas}{Bollob\'as\xspace}
\newcommand{\Furedi}{F\"uredi\xspace}
\newcommand{\Komlos}{Koml\'os\xspace}
\newcommand{\Luczak}{\L uczak\xspace}
\newcommand{\Kucera}{Ku\v{c}era\xspace}
\newcommand{\Szemeredi}{Szemer\'edi\xspace}
\newcommand{\Hastad}{H{\aa}stad\xspace}
\newcommand{\Hoelder}{H\"{o}lder\xspace}
\newcommand{\Holder}{\Hoelder}
\newcommand{\Brandao}{Brand\~ao\xspace}


% {{{ numbersets }}}
% number sets
\newcommand{\Z}{\mathbb Z}
\newcommand{\N}{\mathbb N}
\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\Rnn}{\R_+}
\newcommand{\varR}{\Re}
\newcommand{\varRnn}{\varR_+}
\newcommand{\varvarRnn}{\R_{\ge 0}}


% {{{ problems }}}

% macros to denote computational problems

% use texorpdfstring to avoid problems with hyperref (can use problem
% macros also in headings
\newcommand{\problemmacro}[1]{\texorpdfstring{\textup{\textsc{#1}}}{#1}\xspace}

\newcommand{\pnum}[1]{{\footnotesize #1}}

% list of problems
\newcommand{\uniquegames}{\problemmacro{unique games}}
\newcommand{\maxcut}{\problemmacro{max cut}}
\newcommand{\multicut}{\problemmacro{multi cut}}
\newcommand{\vertexcover}{\problemmacro{vertex cover}}
\newcommand{\balancedseparator}{\problemmacro{balanced separator}}
\newcommand{\maxtwosat}{\problemmacro{max \pnum{3}-sat}}
\newcommand{\maxthreesat}{\problemmacro{max \pnum{3}-sat}}
\newcommand{\maxthreelin}{\problemmacro{max \pnum{3}-lin}}
\newcommand{\threesat}{\problemmacro{\pnum{3}-sat}}
\newcommand{\labelcover}{\problemmacro{label cover}}
\newcommand{\setcover}{\problemmacro{set cover}}
\newcommand{\maxksat}{\problemmacro{max $k$-sat}}
\newcommand{\mas}{\problemmacro{maximum acyclic subgraph}}
\newcommand{\kwaycut}{\problemmacro{$k$-way cut}}
\newcommand{\sparsestcut}{\problemmacro{sparsest cut}}
\newcommand{\betweenness}{\problemmacro{betweenness}}
\newcommand{\uniformsparsestcut}{\problemmacro{uniform sparsest cut}}
\newcommand{\grothendieckproblem}{\problemmacro{Grothendieck problem}}
\newcommand{\maxfoursat}{\problemmacro{max \pnum{4}-sat}}
\newcommand{\maxkcsp}{\problemmacro{max $k$-csp}}
\newcommand{\maxdicut}{\problemmacro{max dicut}}
\newcommand{\maxcutgain}{\problemmacro{max cut gain}}
\newcommand{\smallsetexpansion}{\problemmacro{small-set expansion}}
\newcommand{\minbisection}{\problemmacro{min bisection}}
\newcommand{\minimumlineararrangement}{\problemmacro{minimum linear arrangement}}
\newcommand{\maxtwolin}{\problemmacro{max \pnum{2}-lin}}
\newcommand{\gammamaxlin}{\problemmacro{$\Gamma$-max \pnum{2}-lin}}
\newcommand{\basicsdp}{\problemmacro{basic sdp}}
\newcommand{\dgames}{\problemmacro{$d$-to-1 games}}
\newcommand{\maxclique}{\problemmacro{max clique}}
\newcommand{\densestksubgraph}{\problemmacro{densest $k$-subgraph}}


% {{{ alphabet }}}

\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\cH}{\mathcal H}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

\newcommand{\scrA}{\mathscr A}
\newcommand{\scrB}{\mathscr B}
\newcommand{\scrC}{\mathscr C}
\newcommand{\scrD}{\mathscr D}
\newcommand{\scrE}{\mathscr E}
\newcommand{\scrF}{\mathscr F}
\newcommand{\scrG}{\mathscr G}
\newcommand{\scrH}{\mathscr H}
\newcommand{\scrI}{\mathscr I}
\newcommand{\scrJ}{\mathscr J}
\newcommand{\scrK}{\mathscr K}
\newcommand{\scrL}{\mathscr L}
\newcommand{\scrM}{\mathscr M}
\newcommand{\scrN}{\mathscr N}
\newcommand{\scrO}{\mathscr O}
\newcommand{\scrP}{\mathscr P}
\newcommand{\scrQ}{\mathscr Q}
\newcommand{\scrR}{\mathscr R}
\newcommand{\scrS}{\mathscr S}
\newcommand{\scrT}{\mathscr T}
\newcommand{\scrU}{\mathscr U}
\newcommand{\scrV}{\mathscr V}
\newcommand{\scrW}{\mathscr W}
\newcommand{\scrX}{\mathscr X}
\newcommand{\scrY}{\mathscr Y}
\newcommand{\scrZ}{\mathscr Z}

\newcommand{\bbB}{\mathbb B}
\newcommand{\bbS}{\mathbb S}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbI}{\mathbb I}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbP}{\mathbb P}
\newcommand{\bbE}{\mathbb E}
\newcommand{\bbN}{\mathbb N}

\newcommand{\sfE}{\mathsf E}


% {{{ leqslant }}}
% slanted lower/greater equal signs
\renewcommand{\leq}{\leqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}


% {{{ draftbox }}}
\ifnum\showdraftbox=1
\newcommand{\draftbox}{\begin{center}
  \fbox{%
    \begin{minipage}{2in}%
      \begin{center}%
%        \begin{Large}%
          \Large\textsc{Working Draft}\\%
%        \end{Large}\\
        Please do not distribute%
      \end{center}%
    \end{minipage}%
  }%
\end{center}
\vspace{0.2cm}}
\else
\newcommand{\draftbox}{}
\fi


% {{{ varepsilon }}}

\let\epsilon=\varepsilon

% {{{ numberequationwithinsection }}}
\numberwithin{equation}{section}


% {{{ restate }}}
% set of macros to deal with restating theorem environments (or anything
% else with a label)

% stolen from Boaz's latex macros

\newcommand\MYcurrentlabel{xxx}

% \MYstore{A}{B} assigns variable A value B
\newcommand{\MYstore}[2]{%
  \global\expandafter \def \csname MYMEMORY #1 \endcsname{#2}%
}

% \MYload{A} outputs value stored for variable A
\newcommand{\MYload}[1]{%
  \csname MYMEMORY #1 \endcsname%
}

% new label command, stores current label in \MYcurrentlabel
\newcommand{\MYnewlabel}[1]{%
  \renewcommand\MYcurrentlabel{#1}%
  \MYoldlabel{#1}%
}

% new label command that doesn't do anything
\newcommand{\MYdummylabel}[1]{}

\newcommand{\torestate}[1]{%
  % overwrite label command
  \let\MYoldlabel\label%
  \let\label\MYnewlabel%
  #1%
  \MYstore{\MYcurrentlabel}{#1}%
  % restore old label command
  \let\label\MYoldlabel%
}

\newcommand{\restatetheorem}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{theorem*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{theorem*}
  \let\label\MYoldlabel
}

\newcommand{\restatelemma}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{lemma*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{lemma*}
  \let\label\MYoldlabel
}

\newcommand{\restateprop}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{proposition*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{proposition*}
  \let\label\MYoldlabel
}

\newcommand{\restatefact}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{fact*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{fact*}
  \let\label\MYoldlabel
}

\newcommand{\restate}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \MYload{#1}
  \let\label\MYoldlabel
}


% {{{ bibliography }}}

% add section for references to table of contents
\newcommand{\addreferencesection}{
  \phantomsection
  \addcontentsline{toc}{section}{References}
}


% {{{ mathabbreviations }}}

\newcommand{\la}{\leftarrow}
\newcommand{\sse}{\subseteq}
\newcommand{\ra}{\rightarrow}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\eset}{\emptyset}


% {{{ paragraphperiod }}}


\let\origparagraph\paragraph
\renewcommand{\paragraph}[1]{\origparagraph{#1.}}


% {{{ allowdisplaybreaks }}}
% allows page breaks in large display math formulas

\allowdisplaybreaks


% {{{ sloppy }}}
% avoid math spilling on margin

\sloppy

% {{{ complexityclasses }}}

\newcommand{\cclassmacro}[1]{\texorpdfstring{\textbf{#1}}{#1}\xspace}
\newcommand{\p}{\cclassmacro{P}}
\newcommand{\np}{\cclassmacro{NP}}
\newcommand{\subexp}{\cclassmacro{SUBEXP}}

% {{{ paralist }}}

\usepackage{paralist}

% {{{ comment }}}

\usepackage{comment}


%{{{Bra Ket Notation}}}
\usepackage{braket}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../planted"
%%% End:

